White Paper on Forward Physics, BFKL, Saturation Physics and Diffraction

The goal of this whitepaper is to give a comprehensive overview of the rich field of forward physics. We discuss the occurrences of BFKL resummation effects in special final states, such as Mueller-Navelet jets, jet gap jets, and heavy quarkonium production. It further addresses TMD factorization at low x and the manifestation of a semi-hard saturation scale in (generalized) TMD PDFs. More theoretical aspects of low x physics, probes of the quark gluon plasma, as well as the possibility to use photon-hadron collisions at the LHC to constrain hadronic structure at low x, and the resulting complementarity between LHC and the EIC are also presented. We also briefly discuss diffraction at colliders as well as the possibility to explore further the electroweak theory in central exclusive events using the LHC as a photon-photon collider.

==> header.tex <==

\RequirePackage[colorlinks=true
,urlcolor=blue
,anchorcolor=blue
,citecolor=blue
,filecolor=blue
,linkcolor=blue
,menucolor=blue
,linktocpage=true
,pdfproducer=medialab
,pdfa=true
]{hyperref}

\usepackage{amsmath,amssymb,amsthm,amsfonts}
\usepackage{graphicx,tabularx}
\usepackage{color}
\usepackage{multirow}
\usepackage{comment}
\usepackage{enumitem}
\usepackage{cleveref}
\usepackage{slashed}
\usepackage{float}
\usepackage[normalem]{ulem}
\usepackage{scalerel}
\usepackage{wrapfig}
\usepackage{cancel}
\usepackage{xcolor}
\usepackage[letterpaper,dvips,hmargin={1in,1in},vmargin={1in,1in}]{geometry}

\setlist[description]{leftmargin=0.3cm}
\setlist[itemize]{leftmargin=0.5cm}

\newcommand{\be}{\begin{equation} \begin{aligned}}
\newcommand{\ee}{\end{aligned} \end{equation}}
\newcommand{\bea}{\begin{eqnarray}}  
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}

\def\figureautorefname~#1\null{Fig.\,#1\null}
\def\tableautorefname~#1\null{Tab.\,#1\null}
\renewcommand{\sectionautorefname}{Sec.}
\renewcommand{\subsectionautorefname}{Sec.}
\def\equationautorefname~#1\null{Eq.\,(#1)\null}

% General symbols
\newcommand{\im}{\mathrm{i}}
\newcommand{\diff}{\mathrm{d}}
\newcommand{\eg}{{e.\,g.}~}
\newcommand{\ie}{{i.\,e.}~}
\newcommand{\equivalent}{\simeq}
\newcommand{\br}{\mathrm{BR}}

% Units
\newcommand{\ev}{\text{eV}}
\newcommand{\kev}{\text{keV}}
\newcommand{\mev}{\text{MeV}}
\newcommand{\gev}{\text{GeV}}
\newcommand{\tev}{\text{TeV}}

\newcommand{\ab}{\text{ab}}
\newcommand{\iab}{\text{ab}^{-1}}
\newcommand{\fb}{\text{fb}}
\newcommand{\ifb}{\text{fb}^{-1}}
\newcommand{\pb}{\text{pb}}
\newcommand{\ipb}{\text{pb}^{-1}}

\newcommand{\nm}{\text{nm}}
\newcommand{\micm}{\mu\text{m}}
\newcommand{\mm}{\text{mm}}
\newcommand{\cm}{\text{cm}}
\newcommand{\m}{\text{m}}
\newcommand{\km}{\text{km}}

\newcommand{\mrad}{\text{mrad}}
\newcommand{\murad}{\mu\text{rad}}

\newcommand{\g}{\text{g}}
\newcommand{\kg}{\text{kg}}
\newcommand{\ton}{\text{t}}
\newcommand{\sr}{\text{sr}}
\newcommand{\ns}{\text{ns}}
\newcommand{\hz}{\text{Hz}}

\newcommand{\fasernu}{FASER$\nu$~}

\newcommand{\Eqref}[1]{Equation~(\ref{eq:#1})}
\newcommand{\Eqsref}[2]{Equations~(\ref{eq:#1}) and (\ref{eq:#2})}
\renewcommand{\eqref}[1]{Eq.~(\ref{eq:#1})}
\newcommand{\eqsref}[2]{Eqs.~(\ref{eq:#1}) and (\ref{eq:#2})}
\newcommand{\secref}[1]{Sec.~\ref{sec:#1}}
\newcommand{\secsref}[2]{Secs.~\ref{sec:#1} and \ref{sec:#2}}
\newcommand{\Secref}[1]{Section~\ref{sec:#1}}
\newcommand{\Secsref}[2]{Sections~\ref{sec:#1} and \ref{sec:#2}}
\newcommand{\figref}[1]{Fig.~\ref{fig:#1}}
\newcommand{\figsref}[2]{Figs.~\ref{fig:#1} and \ref{fig:#2}}
\newcommand{\figssref}[3]{Figs.~\ref{fig:#1}, \ref{fig:#2} and \ref{fig:#3}}
\newcommand{\Figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tableref}[1]{Table~\ref{table:#1}}
\newcommand{\tablesref}[2]{Tables~\ref{table:#1} and \ref{table:#2}}
\newcommand{\appref}[1]{Appendix~\ref{sec:#1}}
\newcommand{\appsref}[2]{Appendices~\ref{sec:#1} and \ref{sec:#2}}


%comments
\RequirePackage[normalem]{ulem} 
\newcommand{\changed}[2]{{\protect\color{red}\sout{#1}}{\protect\color{blue}\uwave{#2}}}
%\newcommand{\changed}[2]{#2}
\newcommand{\Felix}[1]{\textcolor{magenta}{[FK: #1]}}
\newcommand{\NOTE}[1]{\textcolor{blue}{ \bf[#1 ]}}
\definecolor{greenST}{RGB}{0,201,87}
\newcommand{\Seb}[1]{\textcolor{greenST}{[ST: #1]}}
\newcommand{\AI}[1]{\textcolor{blue}{[AI: #1]}}
\newcommand{\jlf}[1]{\textcolor{red}{[JLF: {#1}]}}
\newcommand{\gray}[1]{\textcolor{gray}{#1}}
\newcommand{\rem}[1]{\textcolor{magenta}{#1}}
%\newcommand{\rem}[1]{}
\crefname{section}{Sec.}{Secs.}
\crefname{figure}{Fig.}{Figs.}
\crefname{equation}{Eq.}{Eqs.}
\crefname{table}{Table}{Tables}
\crefname{appendix}{Appendix}{Appendices}

%Ref Style
\bibliographystyle{utphys}

\crefname{appendix}{Appendix}{Appendices}
\makeatletter
\def\l@subsubsection#1#2{}
\makeatother

==> tables/neutrino.tex <==
  \begin{tabularx}{\textwidth}{XccCCCCCCCC}
    \toprule
    &
    &
    & \multicolumn{4}{c}{Proton PDF sets}
    & \multicolumn{4}{c}{Nuclear PDF sets}\\
    \midrule
    Data set
    & 
    & Ref.
    & ABMP16
    & CT18
    & MSHT20
    & NNPDF4.0
    & EPPS21
    & nCTEQ15
    & nNNPDF3.0
    & TUJU21
    \\
    \midrule  
    CHORUS $\sigma_{CC}^{\nu,\bar\nu}$
    & Pb
    & \cite{CHORUS:2005cpn}
    & \xmark
    & \xmark
    & \cmark
    & \cmark
    & \cmark
    & \xmark
    & \cmark
    & \cmark
    \\
    CHORUS
    & Pb
    & \cite{Kayis-Topaksu:2011ols}
    & \cmark
    & \xmark
    & \xmark
    & \xmark
    & \xmark
    & \xmark
    & \xmark
    & \xmark
    \\
    NOMAD $\mathcal{R_{\mu\mu}}$
    & Fe
    & \cite{NOMAD:2013hbk}
    & \cmark
    & \xmark
    & \xmark
    & \ymark
    & \xmark
    & \xmark
    & \xmark
    & \xmark
    \\
    CCFR $x F_3^p$
    & Fe
    & \cite{Seligman:1997mc}
    & \xmark
    & \cmark
    & \xmark
    & \xmark
    & \xmark
    & \xmark
    & \xmark
    & \xmark
    \\
    CCFR $F_2^p$
    & Fe
    & \cite{CCFRNuTeV:2000qwc}
    & \xmark
    & \cmark
    & \xmark
    & \xmark
    & \xmark
    & \xmark
    & \xmark
    & \xmark
    \\
    CDSHW $F_2^p, x F_3^p$
    & Fe
    & \cite{Berge:1989hr}
    & \xmark
    & \cmark
    & \xmark
    & \xmark
    & \xmark
    & \xmark
    & \xmark
    & \cmark
    \\
    NuTeV $\sigma_{CC}^{\nu,\bar\nu}$
    & Fe
    & \cite{NuTeV:2001dfo}
    & \cmark
    & \cmark
    & \cmark
    & \cmark
    & \xmark
    & \xmark
    & \cmark
    & \xmark
    \\
    NuTeV $F_2, F_3$
    & Fe
    & \cite{NuTeV:2005wsg}
    & \xmark
    & \xmark
    & \cmark
    & \xmark
    & \xmark
    & \xmark
    & \xmark
    & \xmark
    \\
    \bottomrule
  \end{tabularx}

